Syndrome Decoding of Reed-Solomon Codes Beyond Half the Minimum Distance based on Shift-Register Synthesis

In this paper, a new approach for decoding low-rate Reed-Solomon codes beyond half the minimum distance is considered and analyzed. Unlike the Sudan algorithm published in 1997, this new approach is based on multi-sequence shift-register synthesis, which makes it easy to understand and simple to implement. The computational complexity of this shift-register based algorithm is of the same order as the complexity of the well-known Berlekamp-Massey algorithm. Moreover, the error correcting radius coincides with the error correcting radius of the original Sudan algorithm, and the practical decoding performance observed on a q-ary symmetric channel (QSC) is virtually identical to the decoding performance of the Sudan algorithm. Bounds for the failure and error probability as well as for the QSC decoding performance of the new algorithm are derived, and the performance is illustrated by means of examples.

==> defs.tex <==
\DeclareMathAlphabet{\mathbcal}{OMS}{cmsy}{b}{n}

\DeclareMathOperator{\de2}{d^2_{\mathcal{E}}}
\DeclareMathOperator{\depth}{depth}
\DeclareMathOperator{\wt}{wt}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\length}{length}
\DeclareMathOperator{\neras}{\mathcal{N}}
\DeclareMathOperator{\erfc}{erfc}
\DeclareMathOperator{\sort}{sort}
\DeclareMathOperator{\diag}{diag}

\DeclareMathOperator{\dist}{dist}

\newcommand{\defeq}{\triangleq}

\newcommand{\transp}[1]{\ensuremath{{#1}^\mathsf{T}}}

\newcommand{\Set}[1]{\ensuremath{\left\{{#1}\right\}}}
\newcommand{\SetL}[1]{\ensuremath{\mathcal{#1}}}

\newcommand{\Et}[1]{\ensuremath{\mathcal{E}_t\left({#1}\right)}}
\newcommand{\Vo}[1]{\ensuremath{\mathcal{V}_\omega\left({#1}\right)}}

\newcommand{\ON}[1]{\ensuremath{\mathcal{O}\left({#1}\right)}}

\newcommand{\eras}{\ensuremath{\varepsilon}}

\newcommand{\eproj}[2]{\ensuremath{P_{\neras({#1})}\left[{#2}\right]}}

\newcommand{\set}[1]{\ensuremath{#1}}
\newcommand{\abs}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\vect}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\mat}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\mati}[2]{\ensuremath{\boldsymbol{{#1}_{#2}}}}
\newcommand{\submatr}[3]{\ensuremath{left.\boldsymbol{#1}\right|_{#2}^{#3}}}
%\newcommand{\srt}[1]{\ensuremath{{#1}\!\raisebox{1pt}{$\downharpoonright$}}}
\newcommand{\srt}[1]{\ensuremath{\check{#1}}}

\newcommand{\Wt}[1]{\ensuremath{\wt\left({#1}\right)}}
\newcommand{\Dist}[1]{\ensuremath{\dist\left({#1}\right)}}
\newcommand{\DistE}[1]{\ensuremath{\distE\left({#1}\right)}}
\newcommand{\Dmin}[1]{\ensuremath{\dham\left({#1}\right)}}

\newcommand{\Cu}[1]{\ensuremath{\sigma^{\langle{#1}\rangle}}}
\newcommand{\Ct}{\ensuremath{\Sigma}}

\newcommand{\card}[1]{\ensuremath{\left|{#1}\right|}}
\newcommand{\code}{\ensuremath{\mathcal{C}}}
\newcommand{\codeo}{\ensuremath{\mathcal{A}}}
\newcommand{\codei}{\ensuremath{\mathcal{B}}}
\newcommand{\rscode}{\ensuremath{\mathcal{C}}}
\newcommand{\irscode}{\ensuremath{\boldsymbol{\mathcal{C}}}}
\newcommand{\codeg}{\ensuremath{\mathcal{W}}}
\newcommand{\codet}{\ensuremath{\mathcal{L}}}
\newcommand{\BCH}{\ensuremath{\text{BCH}}}
\newcommand{\RS}[1]{\ensuremath{\mathcal{RS}\left({#1}\right)}}
\newcommand{\Golay}[1]{\ensuremath{\mathcal{G}\left({#1}\right)}}
\newcommand{\IRS}[1]{\ensuremath{\mathcal{IRS}\left({#1}\right)}}
\newcommand{\F}[1]{\ensuremath{\mathbb{F}}_{#1}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\newcommand{\CE}{\ensuremath{\mathcal{E}}}
\newcommand{\FF}[2]{\ensuremath{\mathbb{F}}_{#1}^{#2}}
\newcommand{\GF}[1]{\ensuremath{\text{GF}}\left({#1}\right)}

\newcommand{\Deg}[1]{\ensuremath{\deg\left({#1}\right)}}

\newcommand{\SyS}{\ensuremath{\mathcal{S}}}
\newcommand{\SySi}[1]{\ensuremath{\mathcal{S}^{\left[{#1}\right]}}}
\newcommand{\AuxX}[2]{\ensuremath{{#1}^{\left[{#2}\right]}}}
\newcommand{\SqrX}[2]{\ensuremath{{#1}^{\langle{#2}\rangle}}}
\newcommand{\SuperX}[2]{\ensuremath{{#1}^{\left({#2}\right)}}}
\newcommand{\withl}[2]{\ensuremath{{#1}^{[{#2}]}}}
\newcommand{\Atmaxh}[1]{\ensuremath{\tmax^{\left[{#1}\right]}}}
\newcommand{\Rthh}[1]{R_{\mathrm{th}}^{\left({#1}\right)}}

\newcommand{\Mset}{\ensuremath{\mathcal{S}}}

\newcommand{\ubound}[1]{\ensuremath{\overline{#1}}}
\newcommand{\lbound}[1]{\ensuremath{\underline{#1}}}

\newcommand{\Pfailub}{\ensuremath{\ubound{P}_f}}
\newcommand{\Perrub}{\ensuremath{\ubound{P}_e}}
\newcommand{\Pwrongub}{\ensuremath{\ubound{P}_w}}

\newcommand{\tbmd}{\ensuremath{\tau}}

\newcommand{\nset}{\ensuremath{\mathcal{N}}}
\newcommand{\mset}{\ensuremath{\mathcal{M}}}

\newcommand{\FT}[1]{\ensuremath{\mathscr{F}\left({#1}\right)}}
\newcommand{\IFT}[1]{\ensuremath{\mathscr{F}^{-1}\left({#1}\right)}}

\newcommand{\alg}[1]{\textsf{{#1}}}

\newcommand{\svform}[1]%
{\begin{sideways}\footnotesize\ensuremath{{#1}\;}\end{sideways}}

\newcommand{\algcomment}[1]{\textsf{\footnotesize/$\ast$\ {#1}$\ \ast$/}}

\newcommand{\Oc}[1]{\ensuremath{{\mathcal O}\left({#1}\right)}}

\newcommand{\tmax}{t_{\mathrm{max}}} % tmax general

\makeatletter
\newcommand{\ncirc}[1]{%
        \leavevmode\hbox{\setbox0=\hbox{\ensuremath{#1}}\relax
        \dimen0=\the\wd0\dimen1=\the\ht0
        \ifdim\dimen0>\dimen1\dimen2=\dimen0\else\dimen2=\dimen1\fi
        \divide\dimen0 by 2\divide\dimen1 by 2\advance\dimen2 by 5pt
        \put(\strip@pt\dimen0, \strip@pt\dimen1){\circle{\strip@pt\dimen2}}
        \box0}%
}
\newcommand{\mcirc}[1]{%
        \leavevmode\hbox{\setbox0=\hbox{\scriptsize\ensuremath{#1}}\relax
        \dimen0=\the\wd0\dimen1=\the\ht0
        \ifdim\dimen0>\dimen1\dimen2=\dimen0\else\dimen2=\dimen1\fi
        \divide\dimen0 by 2\advance\dimen0 by -0.4pt
        \divide\dimen1 by 2\advance\dimen1 by -1pt\advance\dimen2 by 1.80pt
        \put(\strip@pt\dimen0, \strip@pt\dimen1){\circle{\strip@pt\dimen2}}
        \box0}%
}
\newcommand{\nbox}[1]{\setlength{\fboxsep}{1.0pt}\fbox{\ensuremath{{#1}}}}
\makeatother

\newcommand{\tmgbox}[1]{\psboxit{box .9 setgray fill}
                     {\setlength{\fboxsep}{1pt}%
                      \spbox{\scriptsize \ensuremath{#1}}}}


==> env.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% env.tex                                                                      %
% created: Apr 14 2000, gs                                                     %
% last changed: Oct 21 2005, gs                                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\theoremstyle{plain}
   \newtheorem{problem}{Problem}}

{\theoremstyle{break}
   \newtheorem{definition}{Definition}}

{\theoremstyle{plain}
   \newtheorem{theorem}{Theorem}}

{\theoremstyle{plain}
   \newtheorem{lemma}{Lemma}}

{\theoremstyle{plain}
   \newtheorem{corollary}[theorem]{Corollary}}

{\theoremstyle{plain}
   \newtheorem{example}{Example}}

